Seeing Eye to AI: Comparing Human Gaze and Model Attention in Video Memorability

Understanding what makes a video memorable has important applications in advertising or education technology. Towards this goal, we investigate spatio-temporal attention mechanisms underlying video memorability. Different from previous works that fuse multiple features, we adopt a simple CNN+Transformer architecture that enables analysis of spatio-temporal attention while matching state-of-the-art (SoTA) performance on video memorability prediction. We compare model attention against human gaze fixations collected through a small-scale eye-tracking study where humans perform the video memory task. We uncover the following insights: (i) Quantitative saliency metrics show that our model, trained only to predict a memorability score, exhibits similar spatial attention patterns to human gaze, especially for more memorable videos. (ii) The model assigns greater importance to initial frames in a video, mimicking human attention patterns. (iii) Panoptic segmentation reveals that both (model and humans) assign a greater share of attention to things and less attention to stuff as compared to their occurrence probability.

==> sections/new_sup_things.tex <==
\input{tables/image_to_video}
\paragraph{Image and video memorability cross-prediction.}
To ascertain the reliability of our simple approach, we evaluate on image memorability tasks (assuming $T{=}1$).
On the LaMem dataset~\cite{khosla_understanding_2015} we match SoTA results (0.720 RC~\cite{squalli2018Lamem}).
On the FIGRIM dataset~\cite{figrim}, we achieve results close to human performance (0.758 RC~\cite{figrim}). \EK{cited paper has 0.74 hor human perfomance}
Previous studies~\cite{Newman2020} pretrain models on image memorability datasets and then fine-tune them for video memorability prediction.
\cref{tab:image_to_video} R2 \vs~R5 shows a small improvement in Memento10k RC score from 0.706 to 0.718 with LaMem pretraining.
However other results do not improve.
We also observe that training on one dataset and evaluating on another (rows 1-4) usually leads to significant degradation and is an important problem for future work.
















\subsection{AUC-Percentile}

For each video frame $f_i$, the true similarity score is computed using AUC-Judd between the model's attention map $\alpha_i$ and the corresponding gaze fixation density map $G_i$.
We then perform a permutation test by comparing the attention map $\alpha_i$ of frame $f_i$ against the fixation map $\hat{G}_i$ from frame $f_i$ of a randomly chosen different video $\hat{V}$. This process is repeated 100 times for each frame, yielding a distribution of 100 AUC-Judd scores under the null hypothesis of no specific relationship between $\alpha_i$ and $\hat{G}_i$. %\PK{VS, is the null hypothesis correctly worded?}\VS{yes}
\MT{this is wrong}
We denote AUC-Percentile for each frame as the percentile of the true similarity score within the distribution of permuted AUC-Judd scores. We compute average over all frames to obtain the AUC-Percentile for a video.
%\MT{PK, VS, reword to center bias argument}
A high AUC-Percentile indicates a strong alignment between the model's attention map and the human gaze fixation density map for the same video, relative to a null distribution of comparisons between different videos. For example, an AUC-Percentile of $80$ implies that there is a less than $20\%$ chance that the observed alignment between the model's attention map and the human gaze fixation density map could be attributed to chance or general center-bias in the data. \MT{why? I don't fully understand this}\VS{better now? It is still unclear though if this method penalizes valid central predictions to a less extent than sAUC in the presence of strong center bias in the data}.
% video $V$ against the fixation map $\hat{G}_i$ from a randomly chosen different video $\hat{V}$ \MT{should above be: of frame $f_i$ against the fixation map $\hat{G}_i$ from frame $f_i$ of a randomly chosen different video $\hat{V}$}.


==> tables/segments.tex <==
\begin{table}[h]
\centering
\small

\begin{tabular}{c c c c c c}
\toprule
Segment & 1 & 2 & 3 & 4 & 5 \\ 
\midrule
RC      & 0.6658 & 0.6785 & 0.6817 & 0.6750 & 0.6560 \\ 
\bottomrule
\end{tabular}
\caption{Correlation scores (RC) for frames sampled from different segments of the video.}
\label{tab:segment_performance}
\end{table}


==> tables/temporal_effects.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\linewidth}{!}{% Adjusts the table to line width
\begin{tabular}{l c cc cc}
\toprule
\multicolumn{2}{c}{} & \multicolumn{2}{c}{Memento} & \multicolumn{2}{c}{Videomem} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
{} & In Seg & RC & MSE & RC & MSE \\ 
\midrule
First & yes & 0.7025 & 0.0061 & 0.5127 & 0.006 \\
Middle & yes & 0.7438 & 0.0051 & 0.5046 & 0.0061  \\
Last & yes & 0.7091 & 0.0056 & 0.5071 & 0.0061 \\
Random & yes & 0.7064 & 0.0061 & 0.5127 & 0.006 \\
First & no & 0.7438 & 0.0051 & 0.5046 & 0.0061  \\
Middle & no & 0.7091 & 0.0056 & 0.5071 & 0.0061 \\
Last & no & 0.7438 & 0.0051 & 0.5046 & 0.0061  \\
Random & no & 0.7091 & 0.0056 & 0.5071 & 0.0061 \\
\bottomrule
\end{tabular}
% }
\caption{Effect of frame picking. Frames chosen within segments versus the entire video.
\TODO{update numbers}}
\label{tab:temporal_effects}
\end{table}



==> tables/text_ablations.tex <==
\begin{table}[t]
\centering
\small
\tabcolsep=0.15cm
% \resizebox{\linewidth}{!}{% Adjusts the table to line width
\caption{Ablation study on using video descriptions.
R1 is the vision-only model for comparison.
We adapt this model to also include captions.
R2 shows that using original captions is beneficial for Memento10k, while jointly predicting captions (R3) only brings a small improvement.}
\label{tab:text_ablation}
\begin{tabular}{ll cc cc}
\toprule
& & \multicolumn{2}{c}{Memento10k (val)} & \multicolumn{2}{c}{VideoMem (val)} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
& Method & RC & MSE & RC & MSE\\ 
\midrule
% No text & \multicolumn{4}{c}{Table 1 row 1} \\
1 & No captions & 0.706 & 0.0061 & 0.513 & 0.0060 \\
2 & w original captions as input  & 0.745 & 0.0050 & 0.505 & 0.0061  \\
% 3 & w orig captions (train) & 0.6492 & 0.0165 & 0.xxx & 0.xxxx  \\
3 & w caption prediction & 0.710 & 0.0056 & 0.508 & 0.0061 \\
\bottomrule
\end{tabular}
% }
% \vspace{2mm}
% \vspace{-5mm}
\end{table}


==> tables/vision_ablations.tex <==
\begin{table}[t]
\centering
\small
\tabcolsep=0.15cm
\caption{Vision ablations.
Column 1 (C1) compares the impact of using spatio-temporal (ST) and temporal (T) features.
C2 and C3 indicate the type of temporal (L: learnable, F: fourier) and spatial position embeddings.
C4 is the frame sampling method.
Best numbers are in \textbf{bold}, second in \textit{italics}.
Row 1 (R1) is chosen as the default configuration for further experiments.
% Spearman Rank Correlation (RC) between ground truth and predictions and Mean square error (MSE) are reported.
}
\label{tab:embeddings_comparison}
% \resizebox{\linewidth}{!}{% Adjusts the table to line width
\begin{tabular}{l c c c c cc cc}
\toprule
& & \multicolumn{2}{c}{Pos. Embedding} & & \multicolumn{2}{c}{Memento10k (val)} & \multicolumn{2}{c}{VideoMem (val)} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& Feature & Time & Space & Sampling & RC & MSE & RC & MSE \\ 
\midrule
1 & ST & F & - & Random & \textbf{0.706} & 0.0061 & \textit{0.513} & \textit{0.0060} \\
\midrule
2 & T & F & - & Random & 0.687 & 0.0062 & 0.508 & 0.0064 \\
3 & ST & L & - & Random & 0.696 & 0.0059 & 0.502 & 0.0060 \\
4 & ST & F & 1D & Random & \textit{0.703} & \textit{0.0057} & 0.506 & \textbf{0.0059} \\
5 & ST & F & 2D & Random & 0.701 & \textbf{0.0056} & 0.505 & \textit{0.0060} \\
6 & ST & F & - & Middle & \textit{0.703} & 0.0066 & \textbf{0.515} & \textbf{0.0059} \\
\bottomrule
\end{tabular}
% }
\end{table}


% \toprule
% \multicolumn{4}{c}{} & \multicolumn{2}{c}{Memento10k} & \multicolumn{2}{c}{VideoMem} \\ 
% \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
% \begin{tabular}[c]{@{}l@{}}Clip\\ Embedding\end{tabular} & \begin{tabular}[c]{@{}l@{}}Temporal\\ Embedding\end{tabular} & \begin{tabular}[c]{@{}l@{}}Position\\ Embedding\end{tabular} & \begin{tabular}[c]{@{}l@{}}Train-time\\ Frames\end{tabular} & RC & MSE & RC & MSE \\ 
% \midrule
% Spatio-temporal & Fourier & None & Random & 0.706 & 0.0061 & 0.513 & 0.0060 \\
% Temporal & Fourier & None & Random & 0.687 & 0.0062 & 0.508 & 0.0064 \\
% Spatio-temporal & Learnable & None & Random & 0.696 & 0.0059 & 0.502 & 0.0060 \\
% Spatio-temporal & Fourier & 1D & Random & 0.703 & 0.0057 & 0.506 & 0.0059 \\
% Spatio-temporal & Fourier & 2D & Random & 0.701 & 0.0056 & 0.505 & 0.0060 \\
% Spatio-temporal & Fourier & None & Middle & 0.703 & 0.0066 & 0.515 & 0.0059 \\
% \bottomrule
% \end{tabular}
% }

